Effective Dimension in Bandit Problems under Censorship

In this paper, we study both multi-armed and contextual bandit problems in censored environments. Our goal is to estimate the performance loss due to censorship in the context of classical algorithms designed for uncensored environments. Our main contributions include the introduction of a broad class of censorship models and their analysis in terms of the effective dimension of the problem -- a natural measure of its underlying statistical complexity and main driver of the regret bound. In particular, the effective dimension allows us to maintain the structure of the original problem at first order, while embedding it in a bigger space, and thus naturally leads to results analogous to uncensored settings. Our analysis involves a continuous generalization of the Elliptical Potential Inequality, which we believe is of independent interest. We also discover an interesting property of decision-making under censorship: a transient phase during which initial misspecification of censorship is self-corrected at an extra cost, followed by a stationary phase that reflects the inherent slowdown of learning governed by the effective dimension. Our results are useful for applications of sequential decision-making models where the feedback received depends on strategic uncertainty (e.g., agents' willingness to follow a recommendation) and/or random uncertainty (e.g., loss or delay in arrival of information).

==> text/old_intro.tex <==
\subsection{Project Review}


\paragraph{Summary:} In the past months, we have started to study sequential decision-making processes under uncertainty, colloquially known as multi-armed bandits, under a broad class of censored environments. Our work is motivated by two types of censorship models: (i) Repeated interaction between a principal and one or more agents where the reception of feedback associated with the principal’s decision (or recommendation) is conditional on the agents' willingness to follow that decision. (ii) Classic and frequent missing data problems where exogenous system faults/failure leads to loss of information and/or delays in arrival of that information. Our goal is to develop improvements to algorithms designed for classical uncensored environments and estimate the performance loss due to censorship. We also aim to arrive at worst-case guarantees on the performance of resulting strategies. This effort contributes to a systematic study of sequential decision making problems in strategic and adversarial environments. 

\paragraph{Motivation:} A typical application is dynamic decision-making in logistics systems where an operator (principal) aims to maximize a cumulative reward metric (e.g. timeliness or fuel usage efficiency) by recommending routes to drivers (agents). At a given time (stage), the principal can only revise estimates on specific routes based on the data from agents who follow its recommendation to take those routes. The choice model of the agents endogenizes the censorship process. Additionally, censorship can also arise due to unreliable or insecure communication between principal and agents. The “optimality” in this decision-making problem depends on how fast the underlying latent condition of the network that governs the stage-wise rewards can be learned. The challenge arises from the fact that the data generating process is mediated by agents’ behavior and the data available is incomplete due to censorship. The question then is to develop efficient algorithms that account for censorship and estimate the performance loss (relative to no censorship benchmark). 

\paragraph{Key Challenge:} Maximizing the cumulative metric of interest in this environment involves balancing between exploring, i.e., learning the unknown payoff relevant parameter, and exploiting the optimal decisions given the current state of knowledge. This duality generates a complex and interdependent sequence of decisions used to both learn and evaluate a posteriori performance. Our ongoing effort is to characterize the impact of censorship on three core features of the problem: the cumulative reward maximization, the learning of the uncertain latent state, and the data generating process. The extensive literature on decision making under uncertainty does not tackle the complex dynamics arising from impact of censorship and the problem is still poorly understood, even for the simplest form of censoring. 

\paragraph{Results:} 
\begin{itemize}
    \item Our main contribution is the introduction and evaluation for a broad class of censorship models of the effective dimension of the problem, a natural measure of its statistical complexity. Intuitively, such effective dimension extends the classical dimension in finite, linear and contextual bandits and governs the magnitude of approximation error in learning and sub-optimality of reward gain w.r.t. clairvoyant player. Interestingly, we show that this effective dimension allows us to maintain the structure of the original problem, while embedding it in a bigger space, and thus to naturally produce comparable results with uncensored settings.
    \item Technically, this involves introducing a new analysis framework culminating in an generalized ellipsoid potential inequality seen through a continuous lens, which we believe is of independent interest due to its wide use by the bandit community. Our proof ideas involve an innovative mix of tools from optimal design, statistical learning and stochastic process theory. Moreover, the worst-case analysis we adopt allows us to precisely understand an adversary’s optimal strategy for negatively influencing learning in the presence of censorship. 
    \item Importantly, we find that such a strategy involves two components whose properties depend on the characteristics of the censorship: (1) an initial transient phase of rapid decay that exploits the misspecification in latent state (e.g. unawareness of censorship), capturing the initial difficulty in the learning task from principal’s perspective; (2) an follow-up stationary phase of slow decay, reflecting the inherent slowdown of learning in the steady state of censored data process.
    % Gauthier: this is of particular importance in fast changing environment where we might never reach the steady state regime.
\end{itemize}
Potential future directions of interest include extending our approach to a more general class of realistic censoring, with particular emphasis on time-dependent processes. Formulating the problem from a Bayesian viewpoint would likely enable to algorithms that extend basic Thompson Sampling (a widely used tool and to gain probabilistic insights on the origin of the effective dimension) to censored environments. We believe that our new perspective can be exploited to design robust algorithms operating efficiently in unknown (and possibly adversarial) environments. 

\subsection{Motivations and Justifications}

In the past months, we have started to study sequential decision-making processes under uncertainty, colloquially known as multi-armed bandits, under a broad class of censored environments. 
Our work is motivated by two types of censorship models:
\paragraph{Setting 1:}Repeated interaction (dynamic decision-making) between a principal and one or more agents where the reception of feedback associated with the principal’s decision (or recommendation) is conditional on the agents' willingness to follow that decision. Use case: Recommender system, A/B testing, Logistics systems.
\paragraph{Setting 2:} Classic and frequent missing data problems in dynamical settings where exogenous system faults/failure leads to loss of information and/or delays in arrival of that information. Use case: Signal processing and control theory, time series analysis, Healthcare, Adaptive Experiments, A/B testing, Transportation, Industry/Economics, Privacy.

\subsection{Literature Review}

==> text/old_pb_setting.tex <==

\subsection{Sequential Online learning: Problem Formulation and Algorithms}

\begin{itemize}
    \item \textbf{Classical Multi-Arm setting/contextual bandits} Our setup involves a principal interacting with an environment over $T$ rounds. The environment depends on an unknown latent parameter $\theta^{\star} \in \Theta \subset \mathbb{R}^{d}$, drawn by Nature. At each round $1,\dots,T$, the principal receives from an oblivious adversary a set of action $\mathcal{A}_{t}$, included in a bounded subset $\mathcal{A}\subset \mathbb{R}^{d}$. From such set, the principal selects an action $a_{t} \in \mathcal{A}_{t}$, according to a strategy $\pi$. To this action will be associated a reward drawn from an action dependent distribution and denoted $y_{a_{t}}\in\mathbb{R}$, modeled in what follows unless notified otherwise as $y\triangleq\langle a,\theta^{\star}\rangle + \epsilon$, where $\epsilon$ is a (conditionally) independent sub-Gaussian Noise of pseudo-variance $\sigma^{2}$. Uncertainty regarding the latent parameter induces uncertainty about the true optimal action at each step $a^{\star}_{t} \triangleq \arg \max_{a\in \mathcal{A}_{t}} \mathbb{E}[y_{a_{t}}]$. Optimal behavior can be expressed in the formalism of Bellman equations, but it is generally intractable, which leads to the study of approximate optimal policies. A surprisingly rich notion to consider is then the  \textit{regret}, the difference in gain between the principal and a clairvoyant agent.  More precisely, we introduce the notion of pseudo-regret:
    \begin{align*}
        R(T)\triangleq \sum_{t=1}^{T} \mathbb{E}[y_{a^{\star}_{t}}-y_{a_{t}}] = \sum_{t=1}^{T} \langle a^{\star}_{t} - a_{t},\theta^{\star}\rangle
    \end{align*}
    where the expectation is with respect to the reward noise only. Performance of different policies are then compared in terms of scaling of the regret with respect to the main quantities of the problem: $T$ the number of rounds and a measure of the \textbf{dimension} of the problem (e.g. number of arm, ambient dimension $d$ or properties of the reward function). One can potentially see this regret through a Bayesian lens by introducing a prior over the possible $\theta^{\star}$ and average over instances of regret. 
    % Gauthier: mention this quickly using the framework from the Paper of Blanchet
    \item \textbf{Censorship and Information Structure}: Uncensored bandits is governed by the filtration $(\mathcal{F}^{NC}_{t})_{t\leq T}$ where $\mathcal{F}^{NC}_{t} \subset \mathcal{F}$ is the sigma algebra generated by $(a_{1},y_{a_{1}},\dots,a_{t-1},y_{a_{t-1}})$. Such action are in turn generated by a possibly randomized policy $\pi\triangleq(\pi_{t})_{t\leq T}$ that is $\mathcal{F}^{NC}_{t}$-adapted. In other word, $\pi_{t}$ can be seen as a distribution probability over actions conditioned by $\mathcal{F}^{NC}_{t}$. 
    One of the key feature of our model is that the reward will not always be observed by the principal. More precisely, it will be observed according to result of a drawn from an action-dependant Bernoulli distribution. In such case, we shall refer to this action as being realized. Such randomness is used to model the choice of the agent in setting $1$ or the potential loss of information in setting $2$. Due to the online setting where the principal endogenously learn about the environment while acting, the design of the information structure is paramount. More precisely, for a given action $a_{t}$, we denote $x_{a_{t}}$ the binary random variable, with value $1$ if and only if the variable was realized. The complete information structure can be defined as the filtration $(\mathcal{F}^{C}_{t})_{t\leq T}$ where $\mathcal{F}^{C}_{t} \subset \mathcal{F}$ is the sigma algebra generated by $(a_{1},y_{a_{1}},x_{a_{1}},\dots,a_{t-1},y_{a_{t-1}},x_{a_{t-1}})$. Let's note $\Pi_{adapt}$ the set of policies time-measurable with respect to this filtration and refer to them as adaptive policies. Yet, we shall first focus on a more realistic setting where reward is observed conditionally on realization and absence of realization i.e. censorship doesn't convey any information. In other words, we shall mainly focus on the filtration $(\mathcal{F}_{t})_{t\leq T}$ where $\mathcal{F}_{t} \subset \mathcal{F}$ is the sigma algebra generated recursively by:
    \begin{align*}
        \mathcal{F}_{t+1}\begin{cases}
      \mathcal{F}_{t}, & \text{if}\ x_{a_{t}}=0 \\
      \mathcal{F}_{t} \cup \sigma(a_{t},y_{a_{t}}), & \text{otherwise}
    \end{cases}
    \end{align*}
    and we shall note $\Pi_{off}\subset \Pi_{adapt}$ the subset of policies time-measurable with respect to this filtration.
    
    \item \textbf{Optimistic algorithms}: In order to study the impact of censorship on the multi-arm problem, this work shall consider the class of high-probability index algorithms based on the \textit{optimism under uncertainty} principle. Beyond the fact that they are widely used in practice, their theoretical study has proven to be intimately linked to that of a larger class of algorithms (notably Thompson Sampling and Information Directed Sampling). More generally, extensions of our techniques can also apply to recent works on non-stationary environments or linear reinforcement learning. The regret analysis of such algorithms relies on two steps: study the average "regret per information gain" achieved by the algorithm at each step and multiply it by the (worst case) total information i.e. maximal uncertainty complexity associated with the problem. 
    % Gauthier: mention the general principle of information directed sampling and the fact that UCB is a class of such algorithm, as well as TS, IDS and co... 
    % Gauthier: quote here the paper 
\end{itemize}
